Physics-driven AI for Channel Estimation in Cellular Network

In cellular mobile networks, wireless channel quality (CQ) is a crucial factor in determining communication performance and user's network experience. Accurately predicting CQ based on real environmental characteristics, specific base station configurations and user trajectories can help network operators optimize base station deployment, improving coverage and capacity. The Received Signal Reference Power (RSRP) and Signal-to-Interference-plus-Noise Ratio (SINR) of user equipment (UE) are key indicators of CQ in wireless communication. However, existing researches have limitations in terms of generation accuracy. Regression methods such as statistical inference and random forests fail to effectively capture the unique characteristics of wireless environments; theoretical derivations relying on specific communication protocols lack generalization capability; data-driven machine learning (ML) methods like Long Short-Term Memory (LSTM) Network often suffer from a lack of interpretability. To overcome these limitations, we propose physics-informed diffusion models, which accurately generate RSRP and SINR at UE based on the wireless environment, base station configurations, and user trajectories. The model adopts a modular and end-to-end design, employing a teacher-student framework to achieve knowledge distillation. This method integrates expert knowledge into the training of diffusion models, enhancing both the interpretability and accuracy, while also facilitating faster convergence of the model parameters. Furthermore, it allows for self-adaptation in various scenarios through few-shot learning. This approach provides valuable guidance for optimizing base station deployment, predicting user network experience, and building real-world simulators.

==> Append.tex <==
{\appendix[Name]

}

==> Rela_Work.tex <==
\section{Related Works}
\subsection{Estimation and Prediction of RSRP and SINR}

\subsection{Diffusion Models}
